Blind Adversarial Network Perturbations

Deep Neural Networks (DNNs) are commonly used for various traffic analysis problems, such as website fingerprinting and flow correlation, as they outperform traditional (e.g., statistical) techniques by large margins. However, deep neural networks are known to be vulnerable to adversarial examples: adversarial inputs to the model that get labeled incorrectly by the model due to small adversarial perturbations. In this paper, for the first time, we show that an adversary can defeat DNN-based traffic analysis techniques by applying \emph{adversarial perturbations} on the patterns of \emph{live} network traffic.

==> channel-decoding.tex <==
% !TEX root = paper.tex

\section{Channel Decoding} \label{sec:channel}

Recently, machine learning, specifically deep learning, has been used in wireless communication applications~\cite{Gruber2017OnDL, 8357902, 8387468, kim2018communication, 8052521}. In this section, we focus on the \textit{channel decoding} task which is the process of converting received messages into information bits in a wireless channel.
Generally, in a wireless communication system, at the transmitter, \textit{k} information bits are encoded into a code of length \textit{N} which is larger than $k$ due to the noisy environment of the channel. Encoded codes are called \textit{codewords} and based on the encoding scheme, codewords have different lengths and different features. The codewords are then modulated using a modulation scheme and transmitted over a noisy channel. After passing through the channel, the receiver demodulates the received signals and decode the information bits from noisy version of codewords. To perform our blind attack in the channel decoding task, we focus on the work done by Gruber et al.~\cite{Gruber2017OnDL}; they use deep learning for one-shot decoding of random and structured codes, and compare the performance and generalization of the decoder with conventional methods on these codes.
Similar to previous scenarios, applying blind adversarial noise in this scenario is more practical, since conventional adversarial examples techniques need to craft the input signal while transmitting over the channel, and this is not feasible, because the input signal reaches the destination before adding the perturbation.
Therefore, we apply our blind attack on the decoding process by adding the adversarial noise to the codewords.

% In wireless communication systems, channel decoding is the process of converting received messages into codewords of a given code. Generally, in a wireless communication, at the transmitter, \textit{k} information bits are encoded into a codeword of length \textit{N}. The codewords are then modulated using a modulation scheme and transmitted over a noisy channel which is usually \textit{Additive White Gaussian Noise (AWGN)} channel. In an AWGN channel, there is a linear addition of wideband or white noise with constant spectral density and a Gaussian distribution of amplitude.
% After passing through the channel, the receiver demodulates the received signals and decode the information bits from noisy version of codewords.
% Recently, deep learning is used to perform the task of decoding in digital communications by learning the behavior of the channel~\cite{}. For instance, Gruber et al.~\cite{} use deep learning for one-shot decoding of random and structured codes, and compare the performance and generalization of the decoder with conventional methods on these codes.
% As we mentioned in section~\ref{}, applying blind adversarial noise in this scenario is more practical, since conventional adversarial examples techniques need to craft the input signal while transmitting over the channel, and this is not feasible, because the input signal reaches the destination before adding the perturbation.
% Therefore, we apply our blind attack on the decoding process by adding the adversarial noise to the codewords.

% In addition to interfere and block the communication, another objective of a Jammer in wireless communication systems is being undetectable. To provide this feature for our blind attack, we force the adversarial noise to resemble a known noise such as Gaussian noise during training of the noise.
% We use the \textit{Moment-Generating Function} properties to achieve this goal. The moment-generating functions of a real-valued random variable $X$ is an alternative specification of its probability distribution and is defined as
% \begin{equation}
%   M_{X}(t) := \mathbf{E}[e^{tX}],\quad  t \in \mathbb{R}
% \end{equation}
%
% \noindent In other words, the moment-generating function is the expectation of the random variable $e^{tX}$.
% An important property of the moment-generating function is that if two distributions have the same moment-generating function, they are identical at almost all points. We use this feature in our training process such that in each iteration we reduce the distance between the empirical moment-generating function of our adversarial noise and a Gaussian distribution which is equal to $e^{\mu{t}}e^{\frac{1}{2}\sigma^2{t^2}}$ for mean $\mu$, and variance $\sigma^2$.


\paragraphb{Attack Setting}
In the real world scenario, the adversarial noise can be generated by a \textit{jammer}, an adversary who tries to interfere or block the wireless communication. The adversary generates a single adversarial noise regardless of the input signal and type of modulation at the transmitter, degrading the decoder performance.
Since the channel decoding is not a classification task, we consider the UT/UF blind attacker who just tries to disrupt and interfere the communication.
We use deep learning based channel decoding method proposed in~\cite{Gruber2017OnDL} as the input model of our attack. Similar to their setting, we use BPSK modulation in an AWGN noisy channel. In an AWGN channel, there is a linear addition of wideband or white noise with constant spectral density and a Gaussian distribution of amplitude.
Both random and structured codes have codeword length $N = 16$ and code rate $r = 0.5$ which means encoding $k = 8$ information bits in the codeword of length $16$.
The adversarial noise has same size as the codewords.
In the training process, the \textit{signal-to-noise-ratio (SNR)} of the AWGN channel noise is constant and equals to $1db$. For testing our attack, we use different values of SNR for the channel noise.
Figure~\ref{fig:cd-setting} shows the setting of our attack in a wireless communication system.
\begin{figure}[!t]
     \centering
     \includegraphics[width = \linewidth]{channel-decoding-setting}
     \caption{Setting of the wireless communication system under blind adversarial attack}
     \label{fig:cd-setting}
\end{figure}

Using the annotations of Algorithm~\ref{alg:general_adv}, we write our objective function as follows:
\begin{align}
  \nonumber J = \Big(\frac{1}{|b_i|} \sum_{x\in b_i} &\mathcal{L}_f \big(f(x+\alpha \times \text{sigmoid}(z) - 0.5), f(x)\big)\Big) \\
   &-C \big(\left\Vert\text{sigmoid}(z)\right\Vert^2 \big)
  % &C_2 \big(\sum_{t\in T}\big(\mathbf{E}[e^{tz}] - e^{\mu{t}}e^{\frac{1}{2}\sigma^2{t^2}}\big)^2 \big) \Big]\Big)
\end{align}

\noindent where $x$ is the the transmitted signal added by the AWGN channel noise.
Similar to image recognition task, our objective function has two components:
First component makes sure that the decoder does not recover the correct information bits.
The second component controls the $l_2$ norm of the perturbation $z$ and makes it as small as possible.
Since sigmoid function takes values in range $(0,1)$, we subtract $0.5$ from the sigmoid function to enable negative values.
% Third component of the loss function force the distribution of the adversarial noise to a Gaussian behavior. We define a set of points $T=\{t_1, t_2, ...,t_n\}$ and for each point we calculate the moment-generating function of our adversarial noise and a Gaussian random variable in these points. Then, we include the distance between these two moment-generating functions in our loss function, and as mentioned earlier in this section, if two random variables have the same moment-generating function in every point, then we can say that they are identical at almost all points.
$C$ is the coefficient to control the effectiveness of each component of the objective function.
We then compare the performance of our blind attacker with the state-of-the-art jamming methods in wireless channels~\cite{jamming}.

\paragraphb{Datasets}
In channel decoding scenario, we deal with man-made signals, therefore, we are able to generate as many training samples as we like. We have $16$ bits codewords and we modulate them using BPSK modulation. Each codeword is corresponded to a specific code.
We can generate test samples by adding random Gaussian noise with length $16$ to modulated codewords. We use batch sizes of 256 for training the adversarial noise and batch sizes of 1000 for testing the attack. The model proposed by Gruber et al. is a fully connected model composed of three hidden layers with ${128, 64, 32}$ number of neurons.

\paragraphb{Results}
We evaluate our attack by obtaining the code of the model proposed by Gruber et al. Based on our evaluations, we set $C$ to $0.1$ and $\alpha$ to $2$. Note that here the power ($l_2$ norm) of the blind adversarial signal defines the strength of our attack.
Our evaluation metric is \textit{Bit Error Rate (BER)} which is the number of bits decoded incorrectly divided by the total number of bits.
We initialize the adversarial noise with a random distribution of mean $0$ and variance $0.01$.
To evaluate our attack, we compare the performance of our method with state-of-the-art jamming techniques in the literature. As suggested by the~\cite{jamming}, when the modulation of the original signal is BPSK, the optimum modulation for jammer is BPSK either.
Therefore, we generate random BPSK signal and add it to the input of the decoder.
As mentioned earlier in this section, Gruber et al. compare the performance of their decoder with both random and structured codes. Note that Gruber et al. use polar structured codes~\cite{polar} to perform their experiments.
Similarly, we perform our attack on both codes either.
Figure~\ref{fig:ber-snr} shows the BER of the channel decoder over different SNR points of noise from $0db$ to $5db$ with different kinds of adversarial noise for random and polar codes. As expected, BPSK jamming and adversarial noise will increase the BER of the decoder. Furthermore, for both random and polar codes, we can see that for an specific SNR point, our adversarial noise increase the BER more than BPSK jamming even with less power. Since the BPSK jamming consists of $\{1,-1\}$ and has a length of $16$, its power ($P_j$) is equal to $4$. However, our adversarial noise will reach worse BER than the optimal jamming with a similar signal power and outperforms the optimum jamming.
\begin{figure}[!t]
    \centering
\begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{ber-snr-random.pdf}
    \caption{Random codes}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{ber-snr-polar.pdf}
    \caption{Polar codes}
\end{subfigure}
\caption{Comparing blind adversarial noise and BPSK jamming with different channel noise SNR. Blind adversarial noise outperforms the optimal jamming in degrading the performance of the decoder for both random and polar codes.}
\label{fig:ber-snr}
\end{figure}


To compare BPSK jamming and adversarial noise with different signal powers, Figure~\ref{fig:ber-power} illustrates the BER of these two attacks over different signal powers. Note that to reduce the power of jammer signal, we randomly makes its components zero to reach different powers.
As can be seen, for both random and polar codes, for all signal powers, adversarial noise is more effective than BPSK jamming and has higher BER.
\begin{figure}[!t]
    \centering
\begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{ber-power-random.pdf}
    \caption{Random codes}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=1.1\linewidth]{ber-power-polar.pdf}
    \caption{Polar codes}
\end{subfigure}
\caption{Comparing blind adversarial noise and BPSK jamming with different signal powers. Blind adversarial noise increase the BER of the decoder more than optimal jammer for different signal powers.}
\label{fig:ber-power}
\end{figure}

% To make the adversarial noise undetectable, we use a property of the moment-generating functions mentioned earlier in this section. We force our adversarial noise to resemble a normal Gaussian distribution by making its moment-generating function close to the normal one in $10$ points, $T=[0,1,2,..,9]$. Based on our experiments, we set the value of $C_2$ to $0.6$ for random codes, and $0.7$ for polar codes.
% Figure~\ref{fig:force-ber} shows the BER of the decoder over different SNR points of the channel noise for both random and polar codes. As expected, our adversarial noise increases the BER of the decoder. However, we can say that the increase in the BER in this case is less than the previous one where there is no effort to make the noise resemble a Gaussian distribution.
% \begin{figure}[!t]
%      \centering
%      \includegraphics[width = 0.8\linewidth]{force-ber-snr.eps}
%      \caption{}
%      \label{fig:force-ber}
% \end{figure}
%
% \noindent To prove that our adversarial noise mimic a Gaussian distribution, we use the Kolmogorov-Smirnov Test~\cite{}. This test can identify whether two samples are drawn from the same distribution.


==> conclusion.tex <==
\section{Conclusions}
We showed that adversarial examples idea can be applied in traffic analysis applications. We argued that normal adversarial example cannot be used and universal (blind) adversarial perturbation are should be used in for online traffic analysis applications. We designed method to craft the blind adversarial perturbations for common feature sets used in traffic analysis applications. 



We also demonstrated blind adversarial perturbations are transferable, therefore, the adversary does not need white-box access to the target model which makes our attacks more important.

We compared the blind perturbations to the traditional perturbation models to attack traffic analysis applications and showed our approach have much better performance. Based on our results, we suggest that traffic analysis works should be evaluated against more adaptive attacks such as our work. 

==> deepcorr.tex <==
% !TEX root = paper.tex

\section{Flow Correlation} \label{sec:deepcorr}
Tor has emerged as the most popular tool to anonymously browse the Internet with more than two million daily users~\cite{dingledine2004tor}. It provides anonymity by relaying
clients' traffic through a series of relays, known as onion-routers, therefore, concealing the correlation between the IP addresses of
the communicating parties (Figure~\ref{}). Tor is a low latency high bandwidth anonymity system. It, however, is not designed to withstand traffic analysis attacks, and it is known to be vulnerable against them. Using deep learning to perform traffic analysis attacks have shown impressive results in deannoymizing Tor communication~\cite{}. In this work, we focus on two different categories of traffic analysis attacks on Tor network. In this section, we introduce the flow correlation attacks and show how we can use blind adversarial perturbations to dismantle their accuracies.




Flow correlation is one of the core techniques used in a broad range of attacks studied against Tor (and other anonymity systems). To perform a flow correlation attack, an observer needs to monitor
 some fraction of flows entering to and exiting from Tor network. The observer, however, does not know if a pair of  ingress (i.e. entering to Tor network) and egress (exiting from Tor network)
 flow is in fact the same flow or they are from different flows~\cite{dingledine2004tor}. Flow correlation methods allow the observer to find the correlation between the ingress and egress flows and deanonymize Tor.


 Nasr et al.~\cite{deepcorr} designed a system called DeepCorr which uses deep learning to perform flow correlation attack on Tor. DeepCorr is currently the state-of-the-art attack and it  outperforms the conventional flow correlation attacks which use statistical correlation metrics.
 DeepCorr uses Inter-Packet Delays (IPDs) and sizes of the packets as the features to learn a correlation function tailored to Tor's complex noisy network. To use a non-blind adversarial example technique, an adversary should add noise to the IPDs and sizes of the packets (by delaying and padding). We argue that using non-blind adversarial example against flow correlation attacks in Tor network is impractical. To craft a non-blind adversary example, the adversary should observe the input which is the network packets and she cannot add noise to them after sending them. Therefore, she needs to buffer all of the packets before computing the non-blind adversarial perturbation, then send the adversarial version of the inputs. Buffering a large number of packets (300 in the case of DeepCorr) before sending, however, cripple Tor connection and make Tor unusable. On the other hand, by using blind adversarial perturbation the adversary already know how  he should  add noise to any packet in a flow in advance.





 In this section, we show that DeepCorr is susceptible to our blind adversarial attack and a blind single adversarial noise can degrade the performance of the DeepCorr drastically. Nasr et al. represented a bidirectional network flow, $i$, using the following structure:
\begin{align}
\nonumber
F_i = [T_{i}^{u};S_{i}^{u};T_{i}^{d};S_{i}^{d}]
\end{align}

\noindent where $T$ is the vector of IPDs of the flow $i$, $S$ is the vector of packet sizes of flow $i$, and the $u$ and $d$ superscripts illustrate "upstream" and "downstream" sides of the flow.
To correlate a pair ingress flows $i$ and egress flow $j$ DeepCorr uses a two-dimensional array composed of 8 rows:
\begin{align}
\nonumber
F(i,j) = [T_{i}^{u};T_{j}^{u};T_{i}^{d};T_{j}^{d};S_{i}^{u};S_{j}^{u};S_{i}^{d};S_{j}^{d}]
\end{align}

\noindent Consequently, we use the above representation for each pair of flow to craft the blind adversarial perturbations.

\paragraphb{Attack Setting}
In the flow correlation application, an adversary uses blind adversarial perturbation as network flow obfuscation mechanisms, e.g., adding delay to the packets or padding dummy data to the packets.
We assume the adversary can only control the first relay (also known as entry relay) between the Tor client and Tor network (in practice, the adversary in this section can be implemented as a bridge~\cite{tor-bridge} in Tor network to defend against flow correlation attacks ). Therefore, she can only add the perturbations to the ingress flow. Moreover, if the adversary perturb the upstream flow (between the client and the entry relay) then the added perturbation propagate through Tor and it will perturb other flows as well. Due to complexity of Tor network, we cannot simulate  the overall effect of perturbing the client upstream. Therefore, to keep our attack realistic and practical we only allow the adversary to add blind adversarial perturbations to the downstream flow between the entry relay and the client which does not directly effect other flows. Also, we only allow small timing perturbations to limit the effect of the downstream traffic on the upstream. Finally, to show the limits of our attack we do not allow the adversary to change the packet sizes and only she can modify the timings. Considering the representation of a network flow mentioned above, the blind adversarial perturbation is added to $T_{i}^{d}$.

Figure~\ref{fig:deepcorr-setting} shows the setting of our attack in DeepCorr flow correlation scenario applied on Tor. Since, flow correlation is a regression task rather than classification, we only consider a UT/UF attacker.
\begin{figure}[!t]
     \centering
     \includegraphics[width = \linewidth]{deepcorr-setting}
     \caption{Setting of the flow correlation scenario under blind adversarial attack}
     \label{fig:deepcorr-setting}
\end{figure}


To control the delay overhead caused by the blind adversarial perturbation, we restrict the mean and standard deviation of our noise to specific values, $\mu$ and $\sigma$ respectively. Moreover, $\mu$ and $\sigma$ defines the strength of the noise. Considering this restriction and using the annotations of Algorithm~\ref{alg:general_adv}, our training objective function can be written as follows:
\begin{align}
\nonumber &J = \Big(\frac{1}{|b_i|} \sum_{x\in b_i} \mathcal{L}_f \big(f(x+\Delta(z)), f(x)\big)\Big), \\
&\Delta(z) = \text{min}(\sigma_z, \sigma)\frac{z - \text{max}(\mu_z - \mu, 0) - \text{min}(\mu_z + \mu, 0)}{\sigma_z}
\end{align}
% \frac{z - max(\mu_z - m, 0) - min(\mu_z + m, 0)}{\sigma_z}
\noindent where $\mu_z$ and $\sigma_z$ are the mean and standard deviation of the blind adversarial noise in each iteration. If the mean or the standard deviation of the adversarial perturbation is larger than $\mu$ and $\sigma$, function $\Delta(.)$ will rescale the perturbation to have the desierd mean and standard deviation. By doing this, we make sure that the added perturbations never exceed our limitations.
%Note that, our blind adversarial perturbations contains negative values which requires buffering of the packets. However, since the blind adversarial delay is precalculated by the blind attacker, buffering is feasible in this scenario.

\paragraphb{Dataset}
We use the DeepCorr dataset containing $2300$ flows for training and $256$ flows for testing. These flows are captured traffic from visited websites using Tor from top Alexa websites.
Similar to~\cite{deepcorr}, to train and test the network, we create a large set of flow pairs including associated flow pairs (flows belonging to the same Tor connection) and non-associated flow pairs (flows belonging to two arbitrary Tor connection). We label an associated flow pair with $1$ and a non-associated flow pair with $0$. In~\cite{deepcorr}, for each captured Tor entry flow, $i$, $N_{neg}$ negative samples are created by forming $F_i^j$ pairs where $j$ is the exit segment of an arbitrary Tor connection.

\paragraphb{Results}
We investigate the impact of our attack on the performance of the DeepCorr in the presence of the blind adversarial perturnations with different strengths.
we set the average of the perturbation  to zero ($\mu =0$) to make sure we do not delay Tor connections. We, however, show the effect of different standard deviations (i.e., $\sigma$) on the performance of correlations attacks.


Figure~\ref{fig:deepcorr-diff-eps} shows the ROC curves of the DeepCorr performance while the flows are delayed based on the learned blind adversarial perturnations using different values of $\sigma$. As expected, increasing the standard deviation of the blind adversarial delay will reduce the accuracy of DeepCorr, such that the blind adversarial delay with standard deviation of $30$ milliseconds reduces the accuracy of DeepCorr from $80\%$ to $33\%$ while having $10^{-4}$ false positive rate which drastically reduce the effectiveness of DeepCorr.
\begin{figure}[!t]
     \centering
     \includegraphics[width = 0.6\linewidth]{deepcorr-diff-eps}
     \caption{Performance of DeepCorr under the blind adversarial attack with different values of $\alpha$. Increasing the standard deviation of the blind adversarial delay reduces the performance of the DeepCorr more drastically.}
     \label{fig:deepcorr-diff-eps}
\end{figure}

 To show how effective the blind adversarial perturbation is, we compare the performance our attack to the case where the added perturbation is from a normal network jitter with the same mean and standard deviation. According to~\cite{}, the network \textit{jitter} in the network follows a Laplacian distribution. We sample a vector of perturbation with the same size of the blind adversarial perturbations for a Laplace distribution with the same mean and variance.

We set the average of both Laplace distribution and adversarial perturbation  $0$ and their standard deviation $30$ milliseconds. Considering this setting, Figure~\ref{fig:deepcorr-compare} shows the ROC curves of DeepCorr while the flows are obfuscated using Laplacian noise and learned adversarial perturbation. As can be seen, the blind adversarial attack outperforms the Laplacian jitter, e.g. with a false positive rate of $10^{-4}$, Laplacian jitter reduces the true positive rate from $80\%$ ot $58\%$, while the blind adversarial delay with the same strength can reduce the true positive rate
to $33\%$. This experiment shows that while DeepCorr is robust against normal network noises it cannot perform well where the adversary crafts a calibrated perturbation to avoid being detected.
\begin{figure}[!t]
     \centering
     \includegraphics[width = 0.6\linewidth]{deepcorr-compare}
     \caption{Performance of DeepCorr under the blind adversarial attack with different values of $\alpha$. Blind adversarial delay outperforms the random Laplacian delay in degrading the performance of the DeepCorr.}
     \label{fig:deepcorr-compare}
\end{figure}


==> image_recon.tex <==
\section{Comparison With Previous work}\label{sec:image}

While our main objective is to generate adversarial examples for the traffic analysis application. In this section, we briefly compare the performance of Algorithm~\ref{alg:general_adv} to Universal adversarial perturbations designed by Moosavi-Dezfooli et al.~\cite{moosavi2017universal} and discuss the improvements of our approach. Universal adversarial perturbations is design for the destination and source untargeted scenario, however, it can be easily modified in 


\paragraphb{Attack Setting}


Blind adversarial perturbations allow the attacker to be independent of input, therefore, she crafts a set of pre-computed filters which when applied to the input device (e.g., camera's lens) force the classifier to misclassify inputs. For example, the attacker can design a translucent filter to put it on the input device lens. In this approach the filter can be made with a very low cost and at scale. Moreover, the attack can be used only on a set of victims.


A translucent filter can only reduce the amount the  light passing through it, this will restrict the adversarial perturbation to only reduce the pixel values (assuming we represent brighter pixels by a higher value). To consider this restriction, we write the loss function as :
\begin{align}
   J =\Big( \frac{1}{|b_i|} \sum_{x \in b_i }  & \mathcal{L}_f (f(\text{min} (x+ \alpha \times \text{sigmoid} (G(z)), 1) ),DT) \Big)
\end{align}

To make sure the adversarial perturbation only reduces light passing through we used sigmoid function~\cite{}, which maps inputs in to the range $(0,1)$ (1 is completely blocking the light for that pixel and 0 no blocking). we used the min function to make sure that when we add the adversarial perturbation to input the combined image does not violate the input space. w.l.o.g, we assumed $1$ is the highest possible value in the input space. Also, $\alpha$ indicate the attacker strength. Larger $\alpha$ results in higher distortion and the filter (i.e. the adversarial perturbation ) will be more visible and vice versa.


\paragraphb{Datasets}


\paragraphbe{MNIST:} We perform experiments on the MNIST image dataset~\cite{deng2012mnist} which consists of 70,000 instances of $28\times28$  handwritten grayscale digit images and the task is to recognize the digits. MNIST splits the training data to 60,000 images for the training and 10,000 for testing phase. We used a convolutional neural network with two convolutional layers and two fully connected layers for the MNIST experiments. We use 5,000 of the testing dataset images to find the blind adversarial examples and other 5,000 to evaluate our attacks.

\begin{figure}
   \begin{subfigure}{0.13\textwidth}
       \centering
       \includegraphics[width=1.\textwidth]{mist_targeted_7_orig_9}
       \caption{Original - 9}
   \end{subfigure}
   \begin{subfigure}{0.13\textwidth}
       \centering
       \includegraphics[width=0.9\textwidth]{mnist_targeted_7}
       \caption{Filter}
   \end{subfigure}
   \begin{subfigure}{0.13\textwidth}
       \centering
       \includegraphics[width=1.\textwidth]{mnist_targeted_7_added_9_7}
       \caption{Classified as 7}
   \end{subfigure}
   \begin{subfigure}{0.5\textwidth}
   \includegraphics[scale=0.13]{mnist_targeted_7_added_0_7}
   \includegraphics[scale=0.13]{mnist_targeted_7_added_1_7}
   \includegraphics[scale=0.13]{mnist_targeted_7_added_2_7}
   \includegraphics[scale=0.13]{mnist_targeted_7_added_3_7}
   \includegraphics[scale=0.13]{mnist_targeted_7_added_4_7}
   \includegraphics[scale=0.13]{mnist_targeted_7_added_5_7}
   \includegraphics[scale=0.13]{mnist_targeted_7_added_6_7}
   \includegraphics[scale=0.13]{mnist_targeted_7_added_8_7}
       \caption{All classified as 7}
   \end{subfigure}





   \caption{Targeted blind adversarial examples on MNIST dataset. Using a single adversarial perturbation which can be applied as a filter to the camera lens inputs from all classes can be classified as the target class which is 7 in this case. For visibility, we flipped the colors of digits. We used $\alpha=0.3$ for this experiment}
   \label{fig:examples_images_mnist}
\end{figure}


 \paragraphb{Results}




\begin{figure*}
\centering
   \begin{subfigure}{0.32\textwidth}
       \centering
       \includegraphics[width=1.\textwidth]{mnist_su_du}
       \caption{SU/DU}
   \end{subfigure}
   \begin{subfigure}{0.32\textwidth}
       \centering
       \includegraphics[width=1.\textwidth]{mnist_st_du}
       \caption{ST/DU}
   \end{subfigure}
   \begin{subfigure}{0.32\textwidth}
       \centering
       \includegraphics[width=1.\textwidth]{mnist_su_dt}
       \caption{SU/DT}
   \end{subfigure}
   \label{fig:mnist_compare}
   \caption{Algorithm~\ref{alg:general_adv} outperforms the previous work~\cite{} in all scenarios. }
\end{figure*}



We evaluated our attacks on  MNIST dataset. Figure~\ref{fig:examples_images_mnist} shows a results of a SU/DT attack on MNIST dataset. The goal of the attack is to make the classifier misclassify any given input as the intended target output class. We choose 7 as our target class for this experiments. As we see in the Figure~\ref{fig:examples_images_mnist}, by adding a single adversarial perturbation, we can make the MNIST classifier to assign label 7 to all given inputs. We used $\alpha =0.3$, 10 epochs, and we used Adam optimizer train the blind adversarial perturbation model with learning rate of 0.0001.  Figure~\ref{fig:mnist_compare} compares the performance of our attack to universal adversarial perturbation in different scenarios. Figures shows that Algorithm~\ref{alg:general_adv} have better performance in training blind adversarial perturbations. Representing the adversarial perturbations as a model allows us to use different optimizer which have a better performance compare to a naive iterative approach. Our main focus is on traffic analysis applications, therefore, we moved more detailed results about our approach on MNIST dataset to Appendix~\ref{app:mnist}.


==> mm <==
This is pdfTeX, Version 3.14159265-2.6-1.40.16 (TeX Live 2015) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./paper.tex
LaTeX2e <2015/01/01>
Babel <3.9l> and hyphenation patterns for 79 languages loaded.
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/size10.clo))
(./usenix2019_v3.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/mathptmx.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/fontenc.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/t1enc.def))
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/inputenc.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/utf8.def
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/t1enc.dfu)
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/ot1enc.dfu)
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/omsenc.dfu)))
(/usr/local/texlive/2015/texmf-dist/tex/latex/pslatex/pslatex.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/sttools/flushend.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/etoolbox/etoolbox.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/color.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/pdftex-def/pdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/ltxcmds.sty)))
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2015/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/hyperref.cfg))

Package hyperref Message: Driver (autodetected): hpdftex.

(/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/breakurl/breakurl.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2015/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))

Package breakurl Warning: You are using breakurl while processing via pdflatex.

(breakurl)                \burl will be just a synonym of \url.
(breakurl)                 on input line 48.

)) (/usr/local/texlive/2015/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/algorithms/algorithmic.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/caption/caption3.sty)))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/graphics.cfg)))
(/usr/local/texlive/2015/texmf-dist/tex/latex/bbm-macros/bbm.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/esvect/esvect.sty)
No file paper.aux.
(/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/omspzccm.fd)
(/usr/local/texlive/2015/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2015/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./paper.out) (./paper.out)
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/ot1ptmcm.fd)
(/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/omlptmcm.fd)
(/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/omxpsycm.fd)
(/usr/local/texlive/2015/texmf-dist/tex/latex/esvect/uesvect.fd)

LaTeX Warning: No \author given.

(./intro.tex

LaTeX Warning: Citation `sirinam2018deep' on page 1 undefined on input line 6.


LaTeX Warning: Citation `deepcorr' on page 1 undefined on input line 6.


LaTeX Warning: Citation `Yoda2000FindingAC' on page 1 undefined on input line 6
.


LaTeX Warning: Citation `RAINBOW' on page 1 undefined on input line 6.


LaTeX Warning: Citation `sirinam2018deep' on page 1 undefined on input line 9.


LaTeX Warning: Citation `deepcorr' on page 1 undefined on input line 11.


LaTeX Warning: Citation `intriguing' on page 1 undefined on input line 15.


LaTeX Warning: Citation `DBLP:journals/corr/GoodfellowSS14' on page 1 undefined
 on input line 15.


LaTeX Warning: Citation `Kurakin2016AdversarialEI' on page 1 undefined on input
 line 15.


LaTeX Warning: Citation `dong2018boosting' on page 1 undefined on input line 15
.


LaTeX Warning: Citation `DBLP:conf/cvpr/Moosavi-Dezfooli16' on page 1 undefined
 on input line 15.


LaTeX Warning: Citation `EAD' on page 1 undefined on input line 15.


LaTeX Warning: Citation `moosavi2017universal' on page 1 undefined on input lin
e 15.


LaTeX Warning: Citation `he2018decision' on page 1 undefined on input line 15.

[1{/usr/local/texlive/2015/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]

LaTeX Warning: Citation `sirinam2018deep' on page 2 undefined on input line 45.



LaTeX Warning: Citation `var-cnn' on page 2 undefined on input line 45.


LaTeX Warning: Citation `deepcorr' on page 2 undefined on input line 45.


LaTeX Warning: Citation `var-cnn' on page 2 undefined on input line 47.


LaTeX Warning: Citation `sirinam2018deep' on page 2 undefined on input line 47.



LaTeX Warning: Citation `deepcorr' on page 2 undefined on input line 48.

) (./threat.tex

LaTeX Warning: Citation `sirinam2018deep' on page 2 undefined on input line 6.


LaTeX Warning: Citation `var-cnn' on page 2 undefined on input line 6.


LaTeX Warning: Citation `rimmer2017automated' on page 2 undefined on input line
 6.


LaTeX Warning: Citation `184463' on page 2 undefined on input line 6.


LaTeX Warning: Citation `panchenko2011website' on page 2 undefined on input lin
e 6.


LaTeX Warning: Citation `cai2012touching' on page 2 undefined on input line 6.


LaTeX Warning: Citation `wang2013improved' on page 2 undefined on input line 6.



LaTeX Warning: Citation `panchenko2016website' on page 2 undefined on input lin
e 6.


LaTeX Warning: Citation `hayes2016k' on page 2 undefined on input line 6.


LaTeX Warning: Citation `wang2016realistically' on page 2 undefined on input li
ne 6.


LaTeX Warning: Citation `deepcorr' on page 2 undefined on input line 6.


LaTeX Warning: Citation `CompressiveTA' on page 2 undefined on input line 6.


LaTeX Warning: Citation `RAINBOW' on page 2 undefined on input line 6.


LaTeX Warning: Citation `chothia2011statistical' on page 2 undefined on input l
ine 6.


LaTeX Warning: Citation `zhu2004flow' on page 2 undefined on input line 6.


LaTeX Warning: Citation `levine2004timing' on page 2 undefined on input line 6.



LaTeX Warning: Citation `shmatikov2006timing' on page 2 undefined on input line
 6.


LaTeX Warning: Citation `houmansadr2014non' on page 2 undefined on input line 6
.


LaTeX Warning: Citation `nasr2017compressive' on page 2 undefined on input line
 6.


LaTeX Warning: Citation `raptor' on page 2 undefined on input line 6.


LaTeX Warning: Citation `RAINBOW' on page 2 undefined on input line 6.


LaTeX Warning: Citation `houmansadr2014non' on page 2 undefined on input line 6
.


LaTeX Warning: Citation `deepcorr' on page 2 undefined on input line 6.


LaTeX Warning: Citation `Yoda2000FindingAC' on page 2 undefined on input line 6
.


LaTeX Warning: Citation `Zhangstep' on page 2 undefined on input line 6.


LaTeX Warning: Citation `deepcorr' on page 2 undefined on input line 18.


LaTeX Warning: Citation `raptor' on page 2 undefined on input line 18.


LaTeX Warning: Citation `var-cnn' on page 2 undefined on input line 19.

[2]

LaTeX Warning: Reference `fig:blind' on page 3 undefined on input line 53.

<./images/blind.pdf, id=21, 412.4208pt x 174.6525pt> <use ./images/blind.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active

LaTeX Warning: Reference `sec:method' on page 3 undefined on input line 90.


LaTeX Warning: Reference `sec:transfer' on page 3 undefined on input line 91.

) (./background.tex [3 <./images/blind.pdf

pdfTeX warning: pdflatex (file ./images/blind.pdf): PDF inclusion: invalid othe
r resource which is no dict (key 'ProcSets', type <array>); ignored.
>]

LaTeX Warning: Citation `vapnik2013nature' on page 4 undefined on input line 23
.


LaTeX Warning: Reference `eq:closs' on page 4 undefined on input line 25.


LaTeX Warning: Citation `goodfellow2016deep' on page 4 undefined on input line 
33.


LaTeX Warning: there is no bold Symbol font on input line 45.


LaTeX Warning: Citation `DBLP:journals/corr/GoodfellowSS14' on page 4 undefined
 on input line 55.


LaTeX Warning: Citation `goodfellow2014explaining' on page 4 undefined on input
 line 55.


LaTeX Warning: Citation `kurakin2016adversarial' on page 4 undefined on input l
ine 55.


LaTeX Warning: Citation `dong2018boosting' on page 4 undefined on input line 55
.


LaTeX Warning: Citation `moosavi2017universal' on page 4 undefined on input lin
e 55.


LaTeX Warning: Citation `DBLP:journals/corr/GoodfellowSS14' on page 4 undefined
 on input line 56.


LaTeX Warning: Citation `kurakin2016adversarial' on page 4 undefined on input l
ine 65.


LaTeX Warning: Citation `dong2018boosting' on page 4 undefined on input line 66
.


LaTeX Warning: Citation `carlini2017towards' on page 4 undefined on input line 
67.


LaTeX Warning: Citation `onepixel' on page 4 undefined on input line 69.


LaTeX Warning: Citation `eykholt2018robust' on page 4 undefined on input line 6
9.


LaTeX Warning: Citation `onepixel' on page 4 undefined on input line 72.


LaTeX Warning: Citation `eykholt2018robust' on page 4 undefined on input line 7
2.


LaTeX Warning: Citation `moosavi2017universal' on page 4 undefined on input lin
e 74.


LaTeX Warning: Citation `CompressiveTA' on page 4 undefined on input line 92.


LaTeX Warning: Citation `RAINBOW' on page 4 undefined on input line 92.


LaTeX Warning: Citation `deepcorr' on page 4 undefined on input line 92.


LaTeX Warning: Citation `bahramali2020' on page 4 undefined on input line 92.


LaTeX Warning: Citation `chothia2011statistical' on page 4 undefined on input l
ine 93.


LaTeX Warning: Citation `zhu2004flow' on page 4 undefined on input line 93.


LaTeX Warning: Citation `levine2004timing' on page 4 undefined on input line 93
.


LaTeX Warning: Citation `shmatikov2006timing' on page 4 undefined on input line
 93.


LaTeX Warning: Citation `houmansadr2014non' on page 4 undefined on input line 9
3.


LaTeX Warning: Citation `nasr2017compressive' on page 4 undefined on input line
 93.


LaTeX Warning: Citation `raptor' on page 4 undefined on input line 93.


LaTeX Warning: Citation `deepcorr' on page 4 undefined on input line 95.

[4]

LaTeX Warning: Citation `sirinam2018deep' on page 5 undefined on input line 102
.


LaTeX Warning: Citation `var-cnn' on page 5 undefined on input line 102.


LaTeX Warning: Citation `rimmer2017automated' on page 5 undefined on input line
 102.


LaTeX Warning: Citation `184463' on page 5 undefined on input line 102.


LaTeX Warning: Citation `panchenko2011website' on page 5 undefined on input lin
e 102.


LaTeX Warning: Citation `cai2012touching' on page 5 undefined on input line 102
.


LaTeX Warning: Citation `wang2013improved' on page 5 undefined on input line 10
2.


LaTeX Warning: Citation `panchenko2016website' on page 5 undefined on input lin
e 102.


LaTeX Warning: Citation `hayes2016k' on page 5 undefined on input line 102.


LaTeX Warning: Citation `wang2016realistically' on page 5 undefined on input li
ne 102.


LaTeX Warning: Citation `rimmer2017automated' on page 5 undefined on input line
 109.


LaTeX Warning: Citation `sirinam2018deep' on page 5 undefined on input line 109
.


LaTeX Warning: Citation `var-cnn' on page 5 undefined on input line 109.


LaTeX Warning: Citation `panchenko2011website' on page 5 undefined on input lin
e 109.


LaTeX Warning: Citation `cai2012touching' on page 5 undefined on input line 109
.


LaTeX Warning: Citation `wang2013improved' on page 5 undefined on input line 10
9.


LaTeX Warning: Citation `panchenko2016website' on page 5 undefined on input lin
e 109.


LaTeX Warning: Citation `hayes2016k' on page 5 undefined on input line 109.


LaTeX Warning: Citation `184463' on page 5 undefined on input line 112.


LaTeX Warning: Citation `panchenko2016website' on page 5 undefined on input lin
e 112.


LaTeX Warning: Citation `hayes2016k' on page 5 undefined on input line 112.


LaTeX Warning: Citation `sirinam2018deep' on page 5 undefined on input line 113
.


LaTeX Warning: Citation `rimmer2017automated' on page 5 undefined on input line
 113.


LaTeX Warning: Citation `var-cnn' on page 5 undefined on input line 113.


LaTeX Warning: Citation `juarez2016toward' on page 5 undefined on input line 11
5.


LaTeX Warning: Citation `wang2017walkie' on page 5 undefined on input line 115.



LaTeX Warning: Citation `cherubin2017website' on page 5 undefined on input line
 115.


LaTeX Warning: Citation `cai2014cs' on page 5 undefined on input line 115.


LaTeX Warning: Citation `sirinam2018deep' on page 5 undefined on input line 115
.


LaTeX Warning: Citation `deepcorr' on page 5 undefined on input line 115.


LaTeX Warning: Citation `juarez2016toward' on page 5 undefined on input line 12
2.


LaTeX Warning: Citation `wang2017walkie' on page 5 undefined on input line 122.



LaTeX Warning: Citation `cherubin2017website' on page 5 undefined on input line
 122.


LaTeX Warning: Citation `cai2014cs' on page 5 undefined on input line 122.


LaTeX Warning: Citation `sirinam2018deep' on page 5 undefined on input line 122
.


LaTeX Warning: Citation `mockingbird' on page 5 undefined on input line 124.

) (./method.tex
Underfull \vbox (badness 2237) has occurred while \output is active

LaTeX Warning: Reference `sec:threat' on page 5 undefined on input line 20.


LaTeX Warning: Reference `eq:adv_main' on page 5 undefined on input line 29.


LaTeX Warning: Citation `moosavi2017universal' on page 5 undefined on input lin
e 37.


LaTeX Warning: Citation `moosavi2017universal' on page 5 undefined on input lin
e 39.


LaTeX Warning: Citation `moosavi2017universal' on page 5 undefined on input lin
e 43.


LaTeX Warning: Citation `hayes2018learning' on page 5 undefined on input line 4
4.


LaTeX Warning: Citation `abdoli2019universal' on page 5 undefined on input line
 44.


LaTeX Warning: Citation `adam' on page 5 undefined on input line 51.


Underfull \hbox (badness 3930) in paragraph at lines 51--54
[]\T1/ptm/m/n/10 We can use ex-ist-ing op-ti-miza-tion tech-niques (e.g.,

LaTeX Warning: Citation `goodfellow2014explaining' on page 5 undefined on input
 line 62.


LaTeX Warning: Citation `kurakin2016adversarial' on page 5 undefined on input l
ine 62.


LaTeX Warning: Citation `dong2018boosting' on page 5 undefined on input line 62
.


LaTeX Warning: Citation `DBLP:journals/corr/GoodfellowSS14' on page 5 undefined
 on input line 62.


LaTeX Warning: Citation `moosavi2017universal' on page 5 undefined on input lin
e 62.

[5]
Overfull \hbox (11.20757pt too wide) in paragraph at lines 91--91
[] 

LaTeX Warning: Reference `eq:erm_untargted' on page 6 undefined on input line 9
4.


Underfull \hbox (badness 10000) in paragraph at lines 94--100
[]\T1/ptm/m/n/10 We ad-just [] for a destination-targeted (\T1/pcr/m/n/10 DT\T1
/ptm/m/n/10 )

Underfull \hbox (badness 10000) in paragraph at lines 94--100
\T1/ptm/m/n/10 at-tack by re-plac-ing $\OT1/ptm/m/it/10 l\OT1/ptmcm/m/n/10 (\OM
L/ptmcm/m/it/10 f\OT1/ptmcm/m/n/10 (\OMS/pzccm/m/n/10 M\OT1/ptmcm/m/n/10 ([]\OM
L/ptmcm/m/it/10 ; G\OT1/ptmcm/m/n/10 (\OML/ptmcm/m/it/10 z\OT1/ptmcm/m/n/10 )))
\OML/ptmcm/m/it/10 ; f\OT1/ptmcm/m/n/10 ([]))$ \T1/ptm/m/n/10 with

Underfull \hbox (badness 1655) in paragraph at lines 94--100
\OMS/pzccm/m/n/10 ^^@\OT1/ptm/m/it/10 l\OT1/ptmcm/m/n/10 (\OML/ptmcm/m/it/10 f\
OT1/ptmcm/m/n/10 (\OMS/pzccm/m/n/10 M\OT1/ptmcm/m/n/10 ([]\OML/ptmcm/m/it/10 ; 
G\OT1/ptmcm/m/n/10 (\OML/ptmcm/m/it/10 z\OT1/ptmcm/m/n/10 )))\OML/ptmcm/m/it/10
 ; O[]\OT1/ptmcm/m/n/10 )$\T1/ptm/m/n/10 , where $\OML/ptmcm/m/it/10 O[]$ \T1/p
tm/m/n/10 is the tar-get out-put

LaTeX Warning: Reference `alg:general_adv' on page 6 undefined on input line 10
3.


LaTeX Warning: Reference `fig:training' on page 6 undefined on input line 103.


LaTeX Warning: Reference `app:scheme' on page 6 undefined on input line 103.


LaTeX Warning: Reference `alg:general_adv' on page 6 undefined on input line 10
4.


LaTeX Warning: Citation `goodfellow2016deep' on page 6 undefined on input line 
106.

) (./perturb.tex

LaTeX Warning: Citation `deepcorr' on page 6 undefined on input line 5.


LaTeX Warning: Citation `var-cnn' on page 6 undefined on input line 5.


LaTeX Warning: Citation `deepcorr' on page 6 undefined on input line 5.


LaTeX Warning: Citation `var-cnn' on page 6 undefined on input line 5.


LaTeX Warning: Citation `sirinam2018deep' on page 6 undefined on input line 5.


LaTeX Warning: Citation `rimmer2017automated' on page 6 undefined on input line
 5.


LaTeX Warning: Citation `184463' on page 6 undefined on input line 5.


LaTeX Warning: Reference `sec:method' on page 6 undefined on input line 21.


Overfull \hbox (8.88048pt too wide) in paragraph at lines 38--38
[] 
[6]

LaTeX Warning: Citation `CompressiveTA' on page 7 undefined on input line 48.


LaTeX Warning: Citation `NIPS2014_5423' on page 7 undefined on input line 50.


LaTeX Warning: Reference `alg:laplace' on page 7 undefined on input line 50.


LaTeX Warning: Reference `alg:size_g' on page 7 undefined on input line 106.


LaTeX Warning: Reference `alg:size_g' on page 7 undefined on input line 107.


LaTeX Warning: Reference `alg:size_g' on page 7 undefined on input line 108.


LaTeX Warning: Reference `alg:size_g' on page 7 undefined on input line 108.


LaTeX Warning: Reference `alg:general_adv' on page 7 undefined on input line 10
8.


LaTeX Warning: Reference `alg:size_g' on page 7 undefined on input line 108.


LaTeX Warning: Reference `alg:size_g' on page 7 undefined on input line 108.


LaTeX Warning: Reference `alg:insert' on page 7 undefined on input line 123.


LaTeX Warning: Reference `alg:insert' on page 7 undefined on input line 124.


LaTeX Warning: Reference `alg:general_adv' on page 7 undefined on input line 12
4.


LaTeX Warning: Reference `alg:insert' on page 7 undefined on input line 124.

[7]

LaTeX Warning: Reference `alg:insert' on page 8 undefined on input line 157.


LaTeX Warning: Reference `eq:grad_where' on page 8 undefined on input line 166.



LaTeX Warning: Reference `alg:grad_v' on page 8 undefined on input line 166.


LaTeX Warning: Reference `alg:grad_v' on page 8 undefined on input line 189.


LaTeX Warning: Reference `eq:grad_where' on page 8 undefined on input line 189.


) (./setup.tex

LaTeX Warning: Citation `paszke2017automatic' on page 8 undefined on input line
 4.


LaTeX Warning: Reference `sec:threat' on page 8 undefined on input line 8.

(/usr/local/texlive/2015/texmf-dist/tex/latex/bbm-macros/ubbm.fd)

LaTeX Warning: Citation `deepcorr' on page 8 undefined on input line 57.


LaTeX Warning: Citation `var-cnn' on page 8 undefined on input line 58.


LaTeX Warning: Citation `sirinam2018deep' on page 8 undefined on input line 58.



Underfull \hbox (badness 1092) in paragraph at lines 57--59
\T1/ptm/m/n/10 Corr [\T1/ptm/b/n/10 ?\T1/ptm/m/n/10 ], and two web-site fin-ger
-print-ing sys-tems, Var-
[8]

LaTeX Warning: Citation `deepcorr' on page 9 undefined on input line 62.


LaTeX Warning: Citation `mockingbird' on page 9 undefined on input line 64.


LaTeX Warning: Citation `var-cnn' on page 9 undefined on input line 87.


LaTeX Warning: Citation `He2015DeepRL' on page 9 undefined on input line 89.


LaTeX Warning: Reference `sec:method' on page 9 undefined on input line 98.


LaTeX Warning: Citation `sirinam2018deep' on page 9 undefined on input line 102
.


LaTeX Warning: Citation `sirinam2018deep' on page 9 undefined on input line 104
.


LaTeX Warning: Citation `juarez2016toward' on page 9 undefined on input line 10
4.


LaTeX Warning: Citation `wang2017walkie' on page 9 undefined on input line 104.



Underfull \vbox (badness 1527) has occurred while \output is active

LaTeX Warning: Citation `sirinam2018deep' on page 9 undefined on input line 114
.


LaTeX Warning: Citation `wang2017walkie' on page 9 undefined on input line 114.



LaTeX Warning: Citation `rimmer2017automated' on page 9 undefined on input line
 114.


LaTeX Warning: Citation `wang2013improved' on page 9 undefined on input line 11
4.


LaTeX Warning: Citation `wang2016realistically' on page 9 undefined on input li
ne 114.


LaTeX Warning: Reference `app:implement' on page 9 undefined on input line 114.



LaTeX Warning: Citation `tor-bridge' on page 9 undefined on input line 119.


LaTeX Warning: Reference `sec:method' on page 9 undefined on input line 125.


LaTeX Warning: Reference `app:params' on page 9 undefined on input line 127.


LaTeX Warning: Reference `sec:method' on page 9 undefined on input line 130.


LaTeX Warning: Reference `sec:method' on page 9 undefined on input line 133.


LaTeX Warning: Reference `app:params' on page 9 undefined on input line 135.

[9]

LaTeX Warning: Citation `deepcorr' on page 10 undefined on input line 141.


LaTeX Warning: Citation `deepcorr' on page 10 undefined on input line 142.


LaTeX Warning: Citation `deepcorr' on page 10 undefined on input line 142.


LaTeX Warning: Citation `sirinam2018deep' on page 10 undefined on input line 14
6.


LaTeX Warning: Citation `rimmer2017automated' on page 10 undefined on input lin
e 146.


LaTeX Warning: Citation `wang2013improved' on page 10 undefined on input line 1
46.


LaTeX Warning: Citation `wang2016realistically' on page 10 undefined on input l
ine 146.

) (./experiments.tex
Underfull \hbox (badness 1248) in paragraph at lines 10--10
[]\T1/ptm/b/n/12 Adversarially Per-turb-ing Packet Di-rec-

LaTeX Warning: Citation `sirinam2018deep' on page 10 undefined on input line 17
.


LaTeX Warning: Citation `sirinam2018deep' on page 10 undefined on input line 17
.


LaTeX Warning: Citation `var-cnn' on page 10 undefined on input line 41.


LaTeX Warning: Citation `var-cnn' on page 10 undefined on input line 41.


LaTeX Warning: Reference `sec:method' on page 10 undefined on input line 60.


LaTeX Warning: Citation `var-cnn' on page 10 undefined on input line 61.


LaTeX Warning: Citation `sirinam2018deep' on page 10 undefined on input line 61
.


LaTeX Warning: Reference `tab:wf_res_deep' on page 10 undefined on input line 6
3.


LaTeX Warning: Reference `tab:wf_res_var' on page 10 undefined on input line 63
.


LaTeX Warning: Reference `sec:method' on page 10 undefined on input line 74.


LaTeX Warning: Citation `deepcorr' on page 10 undefined on input line 74.


LaTeX Warning: Reference `app:params' on page 10 undefined on input line 74.


LaTeX Warning: Reference `fig:deepcorr_timing' on page 10 undefined on input li
ne 78.


LaTeX Warning: Reference `fig:deepcorr_eps' on page 10 undefined on input line 
78.


LaTeX Warning: Reference `fig:deepcorr_mid' on page 10 undefined on input line 
78.

<./images/deepcorr_eps.pdf, id=185, 578.16pt x 433.62pt>
<use ./images/deepcorr_eps.pdf>
<./images/deepcorr_mid.pdf, id=186, 578.16pt x 433.62pt>
<use ./images/deepcorr_mid.pdf>
<./images/deepcorr_eps_lap.pdf, id=187, 578.16pt x 433.62pt>
<use ./images/deepcorr_eps_lap.pdf>

LaTeX Warning: Reference `fig:laplace' on page 10 undefined on input line 104.


LaTeX Warning: Reference `fig:deepcorr_laplace' on page 10 undefined on input l
ine 105.

<./images/laplace.pdf, id=188, 722.7pt x 578.16pt> <use ./images/laplace.pdf>

LaTeX Warning: Citation `var-cnn' on page 10 undefined on input line 117.


LaTeX Warning: Reference `tab:wf_timing_var' on page 10 undefined on input line
 118.

[10] [11 <./images/deepcorr_eps.pdf> <./images/deepcorr_mid.pdf

pdfTeX warning: pdflatex (file ./images/deepcorr_mid.pdf): PDF inclusion: multi
ple pdfs with page group included in a single page
> <./images/deepcorr_eps_lap.pdf

pdfTeX warning: pdflatex (file ./images/deepcorr_eps_lap.pdf): PDF inclusion: m
ultiple pdfs with page group included in a single page
>]

LaTeX Warning: Citation `var-cnn' on page 12 undefined on input line 127.


LaTeX Warning: Citation `var-cnn' on page 12 undefined on input line 127.


LaTeX Warning: Reference `sec:method' on page 12 undefined on input line 150.


LaTeX Warning: Reference `fig:deepcorr_size' on page 12 undefined on input line
 152.

<./images/deepcorr_size.pdf, id=273, 578.16pt x 433.62pt>
<use ./images/deepcorr_size.pdf>
Underfull \vbox (badness 1210) has occurred while \output is active

LaTeX Warning: Reference `tab:wf_res_var_all' on page 12 undefined on input lin
e 167.


LaTeX Warning: Reference `fig:deepcorr_all' on page 12 undefined on input line 
168.


LaTeX Warning: Citation `var-cnn' on page 12 undefined on input line 174.


LaTeX Warning: Citation `var-cnn' on page 12 undefined on input line 174.

<./images/deepcorr_insert.pdf, id=274, 578.16pt x 433.62pt>
<use ./images/deepcorr_insert.pdf>

LaTeX Warning: Citation `juarez2016toward' on page 12 undefined on input line 2
13.


LaTeX Warning: Citation `wang2017walkie' on page 12 undefined on input line 215
.


LaTeX Warning: Citation `sirinam2018deep' on page 12 undefined on input line 21
5.


LaTeX Warning: Citation `var-cnn' on page 12 undefined on input line 218.


LaTeX Warning: Reference `tab:wf_res_var' on page 12 undefined on input line 21
9.

[12 <./images/laplace.pdf> <./images/deepcorr_size.pdf

pdfTeX warning: pdflatex (file ./images/deepcorr_size.pdf): PDF inclusion: mult
iple pdfs with page group included in a single page
> <./images/deepcorr_insert.pdf

pdfTeX warning: pdflatex (file ./images/deepcorr_insert.pdf): PDF inclusion: mu
ltiple pdfs with page group included in a single page
>]

LaTeX Warning: Reference `fig:deepcorr_laplace' on page 13 undefined on input l
ine 221.


LaTeX Warning: Reference `fig:deepcorr_eps' on page 13 undefined on input line 
222.

) (./defense.tex

LaTeX Warning: Citation `kurakin2016adversarial' on page 13 undefined on input 
line 5.


LaTeX Warning: Citation `tramer2017ensemble' on page 13 undefined on input line
 5.


LaTeX Warning: Citation `madry2017towards' on page 13 undefined on input line 5
.


LaTeX Warning: Citation `papernot2016distillation' on page 13 undefined on inpu
t line 5.


LaTeX Warning: Citation `ross2018improving' on page 13 undefined on input line 
5.


LaTeX Warning: Citation `cao2017mitigating' on page 13 undefined on input line 
5.


LaTeX Warning: Reference `fig:l2-hist' on page 13 undefined on input line 16.


LaTeX Warning: Reference `fig:acc-hist' on page 13 undefined on input line 16.

<images/acc-hist.pdf, id=322, 794.97pt x 650.43pt> <use images/acc-hist.pdf>
Underfull \hbox (badness 1735) in paragraph at lines 21--21
[]\T1/ptm/m/n/10 Figure 6: |The ac-cu-racy
<images/l2-hist.pdf, id=323, 794.97pt x 650.43pt> <use images/l2-hist.pdf>

LaTeX Warning: Citation `kurakin2016adversarial' on page 13 undefined on input 
line 35.


LaTeX Warning: Citation `tramer2017ensemble' on page 13 undefined on input line
 35.


LaTeX Warning: Citation `madry2017towards' on page 13 undefined on input line 3
5.


LaTeX Warning: Citation `papernot2016distillation' on page 13 undefined on inpu
t line 35.


LaTeX Warning: Citation `ross2018improving' on page 13 undefined on input line 
35.


LaTeX Warning: Citation `cao2017mitigating' on page 13 undefined on input line 
35.


LaTeX Warning: Citation `madry2017towards' on page 13 undefined on input line 3
7.


LaTeX Warning: Citation `carlini2017adversarial' on page 13 undefined on input 
line 37.

[13 <./images/acc-hist.pdf> <./images/l2-hist.pdf

pdfTeX warning: pdflatex (file ./images/l2-hist.pdf): PDF inclusion: multiple p
dfs with page group included in a single page
>]

LaTeX Warning: Citation `madry2017towards' on page 14 undefined on input line 5
1.


LaTeX Warning: Citation `ross2018improving' on page 14 undefined on input line 
51.


LaTeX Warning: Citation `cao2017mitigating' on page 14 undefined on input line 
51.


Overfull \hbox (11.92091pt too wide) in paragraph at lines 42--54
 [][] 

LaTeX Warning: Citation `madry2017towards' on page 14 undefined on input line 6
8.


LaTeX Warning: Citation `ross2018improving' on page 14 undefined on input line 
68.


LaTeX Warning: Citation `cao2017mitigating' on page 14 undefined on input line 
68.


Overfull \hbox (11.92609pt too wide) in paragraph at lines 59--70
 [][] 

LaTeX Warning: Citation `sirinam2018deep' on page 14 undefined on input line 75
.


LaTeX Warning: Citation `sirinam2018deep' on page 14 undefined on input line 75
.


LaTeX Warning: Citation `ross2018improving' on page 14 undefined on input line 
123.


LaTeX Warning: Citation `papernot2016distillation' on page 14 undefined on inpu
t line 123.


LaTeX Warning: Citation `cao2017mitigating' on page 14 undefined on input line 
127.


LaTeX Warning: Reference `alg:general_adv' on page 14 undefined on input line 1
31.


LaTeX Warning: Reference `alg:defense' on page 14 undefined on input line 131.


LaTeX Warning: Reference `app:def' on page 14 undefined on input line 131.


LaTeX Warning: Reference `tab:defense_wf' on page 14 undefined on input line 13
4.


LaTeX Warning: Reference `tab:defense_deep' on page 14 undefined on input line 
134.


LaTeX Warning: Reference `alg:defense' on page 14 undefined on input line 135.


LaTeX Warning: Citation `sirinam2018deep' on page 14 undefined on input line 14
2.


LaTeX Warning: Citation `sirinam2018deep' on page 14 undefined on input line 14
2.


Overfull \hbox (15.7897pt too wide) in paragraph at lines 145--154
 [][] 

Underfull \hbox (badness 1354) in paragraph at lines 157--157
[]\T1/ptm/m/n/10 Table 11: |Trans-fer-abil-ity of time-

Overfull \hbox (15.7897pt too wide) in paragraph at lines 160--169
 [][] 

Underfull \hbox (badness 1931) in paragraph at lines 172--172
[]\T1/ptm/m/n/10 Table 12: |Trans-fer-abil-ity of size-

Overfull \hbox (15.7897pt too wide) in paragraph at lines 175--184
 [][] 

LaTeX Warning: Citation `ross2018improving' on page 14 undefined on input line 
190.


LaTeX Warning: Citation `papernot2016distillation' on page 14 undefined on inpu
t line 190.

[14]

LaTeX Warning: Citation `cao2017mitigating' on page 15 undefined on input line 
194.


LaTeX Warning: Reference `alg:general_adv' on page 15 undefined on input line 1
98.


LaTeX Warning: Reference `alg:defense' on page 15 undefined on input line 198.


LaTeX Warning: Reference `app:def' on page 15 undefined on input line 198.


Underfull \vbox (badness 2150) has occurred while \output is active

LaTeX Warning: Reference `tab:defense_wf' on page 15 undefined on input line 20
1.


LaTeX Warning: Reference `tab:defense_deep' on page 15 undefined on input line 
201.


LaTeX Warning: Reference `alg:defense' on page 15 undefined on input line 202.

) (./transfer.tex
Underfull \vbox (badness 10000) has occurred while \output is active [15]

LaTeX Warning: Citation `Papernot2016TransferabilityIM' on page 16 undefined on
 input line 11.


LaTeX Warning: Citation `sirinam2018deep' on page 16 undefined on input line 22
.


LaTeX Warning: Citation `rimmer2017automated' on page 16 undefined on input lin
e 22.


LaTeX Warning: Citation `sirinam2018deep' on page 16 undefined on input line 24
.


LaTeX Warning: Reference `tab:transfer_direction' on page 16 undefined on input
 line 24.


LaTeX Warning: Citation `alexnet' on page 16 undefined on input line 29.


LaTeX Warning: Reference `tab:transfer_time' on page 16 undefined on input line
 33.


LaTeX Warning: Reference `tab:transfer_size' on page 16 undefined on input line
 38.

) (./paper.bbl [16]
Underfull \hbox (badness 2376) in paragraph at lines 61--65
\T1/ptm/m/n/10 Web-site fin-ger-print-ing de-fenses at the ap-pli-ca-tion

Underfull \hbox (badness 10000) in paragraph at lines 74--78
[]\T1/ptm/m/n/10 R. Din-gle-dine and N. Math-ew-son.  De-sign

Underfull \hbox (badness 10000) in paragraph at lines 74--78
\T1/ptm/m/n/10 of a Blocking-Resistant Anonymity Sys-tem.

Underfull \hbox (badness 10000) in paragraph at lines 74--78
[][]$\T1/pcr/m/n/10 https : / / svn . torproject . org / svn / projects /

Underfull \hbox (badness 1137) in paragraph at lines 107--110
[]\T1/ptm/m/n/10 Ian J Good-fel-low, Jonathon Shlens, and Chris-tian

Underfull \hbox (badness 4366) in paragraph at lines 143--148
[]\T1/ptm/m/n/10 Amir Houmansadr, Ne-gar Kiyavash, and Nikita

Underfull \hbox (badness 4366) in paragraph at lines 150--154
[]\T1/ptm/m/n/10 Amir Houmansadr, Ne-gar Kiyavash, and Nikita

Underfull \hbox (badness 6461) in paragraph at lines 150--154
\T1/ptm/m/n/10 Borisov.  Non-blind wa-ter-mark-ing of net-work

Underfull \hbox (badness 1348) in paragraph at lines 156--161
[]\T1/ptm/m/n/10 Mohsen Imani, Mo-ham-mad Saidur Rah-man, Nate

Underfull \hbox (badness 3240) in paragraph at lines 156--161
\T1/ptm/m/n/10 Mock-ing-bird: De-fend-ing Against Deep-Learning-
[17]
Underfull \hbox (badness 3229) in paragraph at lines 196--200
[]\T1/ptm/m/n/10 Aleksander Madry, Alek-san-dar Makelov, Lud-wig

Underfull \hbox (badness 1371) in paragraph at lines 286--291
[]\T1/ptm/m/n/10 Payap Siri-nam, Mohsen Imani, Marc Juarez, and
[18]) (./model_details.tex

LaTeX Warning: Reference `tab:model_param' on page 19 undefined on input line 3
.


LaTeX Warning: Reference `fig:training' on page 19 undefined on input line 26.

<./images/training-process.pdf, id=441, 1011.78pt x 304.2567pt>
<use ./images/training-process.pdf>
<./images/end-to-end.pdf, id=442, 469.755pt x 115.3911pt>
<use ./images/end-to-end.pdf>
<./images/end-to-middle.pdf, id=443, 433.62pt x 109.3686pt>
<use ./images/end-to-middle.pdf>

LaTeX Warning: Reference `fig:normal_imp' on page 19 undefined on input line 54
.

) (./defense_mnist.tex

LaTeX Warning: Reference `alg:defense' on page 19 undefined on input line 140.


LaTeX Warning: Reference `alg:general_adv' on page 19 undefined on input line 1
60.

)
! Interruption.
<to be read again> 
                   \flushend@@lastskip@b 
l.173 \end{document}
                    
? 

==> multi_perts.tex <==

\section{Uniqueness Algorithm} \milad{maybe remove if we don't have space}\label{app:uniq}
\begin{algorithm}[h]
\begin{small}
    \caption{Crafting a set of adversarial perturbations}
   \begin{algorithmic}
   	\STATE $\mathcal{D}^{S} \gets$ adversary training data
       \STATE $f \gets$ target model
       \STATE $\mathcal{L}_{f} \gets $ target model loss function
       \STATE $\mathcal{M} \gets$ domain  remapping function
       \STATE $\mathcal{R} \gets$ domain  regularizations function
       \STATE $G(z) \gets$ initialize the blind adversarial perturbation model parameters ($\theta_G$)
       \STATE $T \gets $ epochs
       \STATE DT $ \gets$  the destination target class or false o.w.
       \STATE ST $ \gets$  the source target classes or false o.w.
       \FOR{epoch $t \in \{ 1 \cdots T \}$  }
           \FORALL{mini-batch $b_i$ in $\mathcal{D}^{S}$}
               \IF{ST }
               \STATE $b_i \gets$  select instances only with the ST class label
               \ENDIF
               \STATE $z \sim$ Uniform
               \IF{DT}
               \STATE $J = -(\frac{1}{|b_i|} \sum_{x  \in b_i} \mathcal{L}_{f} (f(\mathcal{M}(x,G(z))),f(x)) ) + \mathcal{R}(G(z)) $
               \ELSE
               \STATE $J = (\frac{1}{|b_i|} \sum_{x  \in b_i, } \mathcal{L}_{f} (f(\mathcal{M}(x,G(z))),\text{DT}) ) + \mathcal{R}(G(z))$
               \ENDIF
               \STATE  Update $G$ to minimize $J$
           \ENDFOR
       \ENDFOR
       \RETURN $G$
       \STATE $\mathcal{D}^{A} \gets$ adversary training data
       \STATE $f \gets$ target model
       \STATE $\mathcal{L}_{f} \gets $ target model loss function
       \STATE $\mathcal{M} \gets$ domain constraints
       \STATE $\delta \gets$ step size
       \STATE $T \gets $ epochs
       \STATE target $ \gets$  the target class or false o.w.
       \STATE focus $ \gets$  the focus class or false o.w.
       \STATE $Z \gets []$ \MCOMMENT{List of adversarial perturbations}
       \STATE $n \gets$ number of adversarial perturbations
       \STATE $C \gets $ regularization constant
       \FOR {$i \in \{ 1 \cdots n\}$ }
       \STATE $z \gets$ initialize the blind adversarial perturbation
        \FOR{epoch $t \in \{ 1 \cdots T \}$  }
            \FORALL{mini-batch $b_i$ in $\mathcal{D}^{A}$}
                \IF{focus}
                \STATE $b_i \gets$  select instances only with the focus class label
                \ENDIF
                \IF{not target}
                \STATE $J = (\frac{1}{|b_i|} \sum_{x  \in b_i} \mathcal{L}_{f} (f(x+z),f(x)) ) - \mathcal{M}(z)$
                \ELSE
                \STATE $J = (\frac{1}{|b_i|} \sum_{x  \in b_i, } \mathcal{L}_{f} (f(x+z),\text{target}) ) - \mathcal{Z}(z) $
                \ENDIF
                \STATE $J = J + C \frac{\sum (Z-z)^2}{|Z|} $
                \STATE  $z =  z + (\delta \times (\nabla J))$
            \ENDFOR
        \ENDFOR
        \STATE Add $z$ to $Z$
       \ENDFOR
       \RETURN $Z$
    \end{algorithmic}
    \label{alg:unique}
\end{small}
\end{algorithm}


==> related.tex <==
\section{Related Works}

==> wf.tex <==
\section{Website Fingerprinting} \label{sec:wf}
In Section~\ref{sec:deepcorr} we introduce Tor and how traffic analysis attacks can deanonymize Tor network. Website fingerprinting is another type of traffic analysis attacks. Several website fingerprinting attacks~\cite{hayes2016k,wang2013improved,wang2016realistically,sirinam2018deep,cai2012touching,cao2017mitigating,panchenko2016website,oh2019p1,rimmer2017automated} have been introduced to undermine anonymity of Tor network. Website fingerprinting allows an attacker to identify web pages in an encrypted connection by analyzing the network traffic.  
In the recent years, researchers showed that it is possible to use deep learning for such attacks~\cite{sirinam2018deep,rimmer2017automated,oh2019p1} which significantly improves the accuracy. Many defenses have  been proposed to make Tor robust against website fingerprinting attack~\cite{juarez2016toward,wang2017walkie,cherubin2017website,cai2014cs}, however, almost all of the are ineffective in practice~\cite{sirinam2018deep}. In this work, we show the feasibility of crafting practical blind adversarial examples which degrade the performance of website fingerprinting attacks drastically. Adversarial examples can be used as a defense against website fingerprinting attacks. To be consistent with the rest of the paper, however, we use ``adversary'' to indicate the entity who uses adversarial example to defeat website fingerprinting in the rest of this section,
 
Website fingerprinting attacks assume an attacker is observing the network traffic between the Tor client and the first relay (also known as entry relay). To apply the adversarial examples against website fingerprinting attacks in this setting, a client and its entry relay should change the traffic pattern. Similar to the flow correlation attacks, using non-blind adversarial example is not practical. In a non-blind adversarial example attack, the client and relay should have the traffic pattern to use it in a non-blind adversarial example algorithm this means that they need to buffer a large number of packets to generate the input (about 5,000 packets~\cite{sirinam2018deep}) which delays all communication and extremely slows them down. Even if an attack requires smaller number of packets to craft the adversarial examples it should run a complex neural network which takes up to several milliseconds~\cite{} which again delay the connection. Blind adversarial examples allows us to a set of pre-computed perturbations which can be applied in the runtime regardless of the inputs.


\paragraphb{Attack Setting}
In particular, we focus on the recent work of Sirinam et al.~\cite{sirinam2018deep}. They designed a complex convolutional neural network for this task. This work does not train on the raw features instead for a given network traffic flow they extract the packet's directions as  features  and use them to train their website fingerprinting model. They assume each traffic flow has 5,000 packets which is  represented by a vector with 5000 elements each element is, $1$, if the client is the packet sender and, $-1$, if the relay is the sender. Having  binary input space makes crafting adversarial examples challenging while more interesting. Therefore, we generate a custom attack algorithm for this application.
 
In this application, we assume adversary can only append a limited set of packets to the communication between the client and relay and she does not want to delay any packets tp avoid slowing  down Tor connections. We define $\alpha$ to indicate the adversary's strength which is the number of packets that she is allowed to inject to a traffic flow. We assume the adversary knows the input size of website fingerprinting model (5,000 in this case). The adversary wants to use blind adversarial perturbation method to find  a set of  $\alpha$ positions and the directions which then she will append packets based on that. In  practice, We also assume the client and relay agree on a set of pre-computed perturbations and if the perturbation indicates to  inject a packet at position $i$, the client or relay send a dummy packet. Please note that Tor encrypts all of communication so an observer cannot distinguish between dummy and genuine packets. To make this adversarial attack more practical, we assume when the adversary insert a packet at position $i$ all of original packet from position $i$ to the end of the flow will shift by one. Therefore, the adversary does not need to direction of any existing packet (which is impractical).
 
We design a custom activation layer for this purpose which we denote by $\Gamma(x,z,\alpha)$. Our activation layer $\Gamma$ gets a feature vector ($x$) (extracted from a network traffic flow), the adversarial perturbation which we represent by  a float vector with the same dimension as feature vector ($z$), and the adversary's strength ($\alpha$). In a nutshell, this layer selects the $\alpha$  positions from the perturbation vector where the elements has the highest absolute values, then it inserts an element at the selected positions  $-1$ if the value of perturbation is less than zero and $1$ otherwise (and shift the consequent packets), and trim the vector to have the same size of original flow (i.e., $x$) .Appendix~\ref{} explains  details about this layer and how we back-propagate gradients.
 
 
Finally we write the objective function for compute the adversarial perturbation as follows:
\begin{align}
   J =\Big( \frac{1}{|b_i|} \sum_{x \in b_i }  & \mathcal{L}_f (f(\Gamma(x,z,\alpha)),f(x)) \Big)
\end{align}
 
 
The activation layer $\Gamma$ makes sure that the generate adversarial example is with in the input data dimension.
 
 
 
\paragraphb{Datasets}
We used the Tor network traces' dataset  provided by Sirinam et al.~\cite{sirinam2018deep}. The dataset consists of 95,000 network traffic flow from  95 classes (each class represents a website) with 1,000 flows for each. They extracted  Tor cell's direction in the traffic flows. They assume each flow has 5,000 Tor cells (they padded or truncated shorter or longer flows.).  We used 7,000 instances for training, 1,000 instances for validation, and 1,500 instances for testing.
 
 
\paragraphb{Results}
 
 
\begin{table*}
   \centering
   \caption{The attack accuracy for different attack settings on website fingerprinting work proposed by~\cite{sirinam2018deep}, the model has $92\%$  accuracy. }
   \resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllllll@{}}
    \toprule
$\alpha$ &Bandwith Overhead ($\%$) & UT/UF  ($\%$) & Max UT/F (\#, $\%$)  & Min UT/F  (\#, $\%$) & Max T/UF (\#, $\%$) & Min T/UF (\#, $\%$) & Max T/F (\#$\leftarrow $\#, $\%$) & Min T/F (\#$\leftarrow $\#, $\%$)\\
\midrule  
20 & 0.04 & $24.2 $  & $-, 100.0$ & $-, 0.0$     & $77, 31.9$  & $4, 0.1$  &  $-, 100.0$  & $-, 0.0 $  \\
%30 & 0.06 &$31.4$  & $-, 100.0$ & $-, 0.0$     & $59, 41.2$ & $40, 1.4$  &  $-, 100.0$  & $-, 0.0 $  \\
%50 & 1.01 &$40.0$ & $-, 100.0$ & $-, 0.0$  & $74, 52.8$ & $47, 4.8$ &  $-, 100.0$ & $-, 0.0 $  \\
100 & 2.04 &$49.6 $ & $-, 100.0$ & $47, 0.0$ & $34, 77.6$ & $89, 13.2$ &  $-, 100.0$     & $-, 0.0 $ \\
%200 & 4.16 &$69.8 $ & $-, 100.0$ & $69, 2.0$ & $58, 87.2$& $43, 20.8$ &  $-, 100.0$     & $-, 0.0 $  \\
500 & 11.11 &$91.8 $ & $-, 100.0$ & $49, 4.0$ & $92, 97.1$& $82, 47.8$ &  $-, 100.0$   & $23\leftarrow 69, 0.1 $  \\
1000 & 25.0 & $95.7 $ & $-, 100.0$ & $21, 29.0$ & $-, 100.0$& $10, 67.0$ &  $-, 100.0$   & $72\leftarrow 47, 4.4 $  \\
2000 & 66.66 & $97.7 $ & $-, 100.0$ & $48, 94.7$ & $-, 100.0$& $37, 89.4$ &  $-, 100.0$   & $78\leftarrow 60, 35.4 $  \\
\bottomrule
\end{tabular}}
\label{tab:wf_res}
\end{table*}
 
We evaluated our attack for different adversary settings and strengths. We used 10 epochs and $\delta = 0.02$ to craft the blind adversarial perturbations. Table~\ref{tab:wf_res}, shows the results of our attack. We found several websites where with very small perturbations the network observer (who is deploying the website fingerprinting attack) misclassify them (focused attacks). Moreover, in the targeted attacks, the blind adversary can generate adversarial perturbations which makes the classifier misclassify every input as the targeted class with only 25.0 $\%$ overhead.
 
We compared our results with the proposed counter-attcks against website fingerprinting methods. Juarez et al.~\cite{juarez2016toward} proposed WTF-PAD which adaptively add dummy packets to Tor traffic to evade website fingerprinting attacks. Using WTF-PAD on this dataset have 64$\%$ bandwidth overhead and make reduce the detection accuracy to $3\%$, while using targeted blind adversarial attack (with several possible targets) with only 25$\%$ bandwidth overhead it can reduce the detection accuracy to $1\%$ which is similar to a random guess. Similarly, using the defense proposed by Wang and Goldberg called Walkie-Talkie~\cite{wang2017walkie}, the detection accuracy decrease to $5\%$ with $31\%$ bandwidth overhead and $36\%$ latency overhead~\cite{sirinam2018deep}. Please keep in mind that our approach does not delay any packet and only inject packets and similar to WTF-PAD does not have latency overhead.
 
 
In this paper, we focus on showing the feasibility of the blind adversarial attacks against website fingerprinting methods. While we showed impressive results,  a comprehensive study is still required to investigate and analyze the behavior of the blind adversarial perturbations. For example, as shown in Table~\ref{tab:wf} some websites are much easier to imitate (as a target) or to change (as a focus). Investigate such inconsistency can give reveal interesting properties which can be used later to design more effective attacks and defense. Unfortunately, such analyses are beyond the scope of this paper.
 




